ESPnet-ST-v2: Multipurpose Spoken Language Translation Toolkit

ESPnet-ST-v2 is a revamp of the open-source ESPnet-ST toolkit necessitated by the broadening interests of the spoken language translation community. ESPnet-ST-v2 supports 1) offline speech-to-text translation (ST), 2) simultaneous speech-to-text translation (SST), and 3) offline speech-to-speech translation (S2ST) -- each task is supported with a wide variety of approaches, differentiating ESPnet-ST-v2 from other open source spoken language translation toolkits. This toolkit offers state-of-the-art architectures such as transducers, hybrid CTC/attention, multi-decoders with searchable intermediates, time-synchronous blockwise CTC/attention, Translatotron models, and direct discrete unit models. In this paper, we describe the overall design, example models for each task, and performance benchmarking behind ESPnet-ST-v2, which is publicly available at https://github.com/espnet/espnet.

==> tables/data.tex <==
\resizebox {\linewidth} {!} {
\begin{tabular}{lcccccc}
\toprule
Dataset & Task & Source Lang(s) & Target Lang(s) & Domain & \# Train/Valid/Test Utts & \# Speech Train Hours \\
\midrule
IWSLT17 \cite{cettolo2012wit3} & MT & De & En & TED Talk & 160k/7k/7k & - \\
IWSLT17 \cite{cettolo2012wit3} & MT & De & Es & TED Talk & 160k/7k/7k & - \\
\midrule
MuST-C-v2 \cite{di-gangi-etal-2019-must} & ASR/ST & En & De & TED Talk & 250k/1k/3k & 450h \\
MuST-C-v2 \cite{di-gangi-etal-2019-must} & ASR/ST & En & Ja & TED Talk & 330k/1k/3k & 540h \\
\midrule
MTedX \cite{salesky2021multilingual} & MT & Es, Fr, Pt, It, Ru, El & En & TED Talk & 130k/6k/6k & -  \\
MTedX \cite{salesky2021multilingual} & ASR & Es, Fr, Pt, It, Ru, El & En & TED Talk & 400k/6k/6k & 730h \\
MTedX \cite{salesky2021multilingual} & ST & Es, Fr, Pt, It, Ru, El & En & TED Talk & 130k/6k/6k & 250h \\
\midrule
EuroParl \cite{iranzo2020europarl} & MT & De & En & Parliament Speech & - /-/2k & - \\
EuroParl \cite{iranzo2020europarl} & ST & En & De & Parliament Speech & -/-/1k & -\\
\bottomrule
\end{tabular}
}

==> tables/offline_lang.tex <==
\resizebox {.7\linewidth} {!} {
\begin{tabular}{l|ccccccccc}
\toprule
& \multicolumn{9}{c}{MuST-C} \\
& DE & ES & FR & IT & NL & PT & RO & RU & avg. \\
\midrule
NeurST Attentional Enc-Dec & 22.8 \\
Fairseq Attentional Enc-Dec & 22.7 \\
ESPnet-ST Attentional Enc-Dec & 22.9 \\
\midrule
\textbf{\textit{ESPnet-ST-v2}} \\
CTC/Attention + HIC + SAI & 28.8 & 2/20 & 2/18 & 2/20 & 2/20 & 2/20 & 2/22 & 2/22 \\
\bottomrule
\end{tabular}
}


==> tables/s2st_lang.tex <==
\resizebox {\linewidth} {!} {
\begin{tabular}{l|c|cccc|cccccc}
\toprule
System & Avg & fr & de & ca & es & fa & it & ru & zh & pt & nl \\
\midrule
Translatotron* & 3.4 &  \\
Translatotron2* \\
\midrule
\textbf{\textit{ESPnet-ST-v2}} \\
Unity \\
\bottomrule
\end{tabular}
}
